Capacitive displacement method to determine the longitudinal piezoelectric coefficients of single crystals, ceramics and thin films

Recent developments in piezoelectric films have heightened the need for the reliable methods to correctly characterize their piezoelectric coefficients. Here, we demonstrate that capacitive displacement method can be used to determine longitudinal piezoelectric coefficients in both bulk and thin film of piezoelectric materials reliably and simply. Our technique allows accurate detection of elastic displacement at a level of 2 pm. This achievement is of great interest and significance for the development of piezoelectric integration technology in modern smartdevices.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

